Generating Complete and Finite Test Suite for ioco: Is It Possible?

Testing from Input/Output Transition Systems has been intensely investigated. The conformance between the implementation and the specification is often determined by the so-called ioco-relation. However, generating tests for ioco is usually hindered by the problem of conflicts between inputs and outputs. Moreover, the generation is mainly based on nondeterministic methods, which may deliver complete test suites but require an unbounded number of executions. In this paper, we investigate whether it is possible to construct a finite test suite which is complete in a predefined fault domain for the classical ioco relation even in the presence of input/output conflicts. We demonstrate that it is possible under certain assumptions about the specification and implementation, by proposing a method for complete test generation, based on a traditional method developed for FSM.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{A. Petrenko, H. Schlingloff (Eds.): Ninth Workshop on \\
Model-Based Testing (MBT 2014)\\
EPTCS 141, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.141.5}{10.4204/EPTCS.141.5}}
\pdfoutput=1

